Study of $\Upsilon(10753)$ decays to $\pi^{+}\pi^{-}\Upsilon(nS)$ final states at Belle II

We present an analysis of the process $e^{+}e^{-}\to\pi^{+}\pi^{-}\Upsilon(nS)$ (where $n$ = 1, 2, or 3) reconstructed in $19.6\rm$ $\rm fb^{-1}$ of Belle II data during a special run of the SuperKEKB collider at four energy points near the peak of the $\Upsilon(10753)$ resonance. By analyzing the mass distribution of the $\pi^+\pi^-\Upsilon(nS)$ system and the Born cross sections of the $e^{+}e^{-}\to\pi^{+}\pi^{-}\Upsilon(nS)$ process, we report the first observation of $\Upsilon(10753)$ decays to the $\pi^{+}\pi^{-}\Upsilon(1S)$ and $\pi^{+}\pi^{-}\Upsilon(2S)$ final states, and find no evidence for decays to $\pi^{+}\pi^{-}\Upsilon(3S)$. Possible intermediate states in the $\pi^+\pi^-\Upsilon(1S,2S)$ transitions are also investigated, and no evidence for decays proceeding via the $\pi^\mp Z_b^\pm$ or $f_0(980)\Upsilon(nS)$ intermediate states is found. We measure Born cross sections for the $e^{+}e^{-}\to\pi^{+}\pi^{-}\Upsilon(nS)$ process that, combined with results from Belle, improve the precision of measurements of the $\Upsilon(10753)$ mass and width by nearly a factor of two to $(10756.3\pm2.7\pm0.6)$ MeV/$c^2$ and $(29.7\pm8.5\pm1.1)$ MeV, respectively. The relative ratios of the Born cross sections at the $\Upsilon(10753)$ resonance peak are also reported for the first time.

==> authors.tex <==
%%% Paper:    Y(10753) to pi pi Y(nS)
%%% Journal:  JHEP
%%% Contacts: B. Fulsom, J. Yin
%%% ====================================================================
%%% Use \input{pub037} to insert this material into your latex file.
\newcounter{AffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSinica{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCPPM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYerevan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGoettingen{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instBeihang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBINP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCinvestavIPN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPrague{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChiangMai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChiba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChonnam{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChula{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instConacyt{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDESY{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDuke{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instITAR{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instJuelich{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFuJen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFudan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGifu{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSOKENDAI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMainz{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGyeongsang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHanyang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHeidelberg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKEK{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJPARC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHiroshima{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHUNNU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIKERBASQUE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFrascati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIISER{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITBhubaneswar{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITGuwahati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITHyderabad{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITJodhpur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITMadras{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIndiana{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPRussia{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHEPHYVienna{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPChina{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChennai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIOP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIFIC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instISU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJAEA{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJLU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKarlsruhe{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKitasato{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKISTI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKoreaUnivKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyotoU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyungpook{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGiessen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLuther{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMNITJaipur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMcGill{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMETU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMEPhI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoya{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNagoyaIAR{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoyaKMI{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNNU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNankai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNaraWu{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUNAM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHSE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNTUTaiwan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNUUTaiwan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKrakow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNiigata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instOkinawa{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instOsakaMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRCNP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPNNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjab{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instPeking{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMPP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMPGHLL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjabPAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRIKENMSL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSeoul{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instShandong{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyiv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSPU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoochow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoongsil{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSEU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaJSI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSKKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTelAviv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instToho{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTohoku{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTitech{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTokyoMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUAS{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteUNIV{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMontreal{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIJCLab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPHC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instAdelaide{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instBilbao{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBonn{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUBC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCincinnati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFlorida{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHamburg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHawaii{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUniLJ{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLouisville{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMalaya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instManitoba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMelbourne{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMississippi{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUOM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNovaGorica{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUPES{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPittsburgh{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUSTC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSAlabama{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSCarolina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSydney{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTabuk{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUTokyo{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instEri{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVictoria{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUppsala{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVPI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instWayneState{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instXavier{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYamagata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYonsei{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instZZU{\protect\theAffiliationCounter}
\collaboration{The Belle II Collaboration}
% \author[\instTriesteINFN]{F.~Abudin{\'e}n,} % 2250
  \author[\instKEK,\instSOKENDAI]{I.~Adachi,} % 2590
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{K.~Adamczyk,} % 2239
  \author[\instPanjab]{L.~Aggarwal,} % 10083
% \author[\instBonn]{P.~Ahlburg,} % 2367
  \author[\instXavier]{H.~Ahmed,} % 11323
% \author[\instKoreaUnivKU]{J.~K.~Ahn,} % 7423
  \author[\instUTokyo]{H.~Aihara,} % 2223
  \author[\instYerevan]{N.~Akopov,} % 9443
  \author[\instNapoliUNIV,\instNapoliINFN]{A.~Aloisio,} % 2194
% \author[\instMPGHLL]{L.~Andricek,} % 2098
  \author[\instIOP]{N.~Anh~Ky,} % 2218
  \author[\instBNL]{D.~M.~Asner,} % 4684
  \author[\instCincinnati]{H.~Atmacan,} % 2538
% \author[\instBINP,\instNSU]{V.~Aulchenko,} % 8183
  \author[\instHSE]{T.~Aushev,} % 3747
  \author[\instKyiv]{V.~Aushev,} % 2155
  \author[\instNagoya]{M.~Aversano,} % 7363
% \author[\instTata]{T.~Aziz,} % 3523
  \author[\instIPHC]{V.~Babu,} % 5623
% \author[\instKrakow]{S.~Bacher,} % 2258
  \author[\instUTokyo]{H.~Bae,} % 10863
  \author[\instIITBhubaneswar]{S.~Bahinipati,} % 2332
% \author[\instSydney]{A.~M.~Bakich,} % 2115
  \author[\instIJCLab]{P.~Bambade,} % 3003
  \author[\instLouisville]{Sw.~Banerjee,} % 8603
  \author[\instPanjab]{S.~Bansal,} % 5163
  \author[\instKEK]{M.~Barrett,} % 2180
% \author[\instPisaUNIV,\instPisaINFN]{G.~Batignani,} % 6643
  \author[\instIPHC]{J.~Baudot,} % 2562
% \author[\instKarlsruhe]{M.~Bauer,} % 9863
  \author[\instDESY]{A.~Baur,} % 5683
  \author[\instVictoria]{A.~Beaubien,} % 6683
  \author[\instDESY]{F.~Becherer,} % 21623
  \author[\instKarlsruhe]{J.~Becker,} % 5403
% \author[\instIITMadras]{P.~K.~Behera,} % 4204
  \author[\instMississippi]{J.~V.~Bennett,} % 2454
% \author[\instRomaTreINFN]{E.~Bernieri,} % 4483
  \author[\instBonn]{F.~U.~Bernlochner,} % 2282
  \author[\instCPPM]{V.~Bertacchi,} % 2212
  \author[\instBNL]{M.~Bertemes,} % 2595
  \author[\instTelAviv]{E.~Bertholet,} % 13163
  \author[\instHawaii]{M.~Bessner,} % 3783
  \author[\instPisaUNIV,\instPisaINFN]{S.~Bettarini,} % 2350
% \author[\instIISER]{V.~Bhardwaj,} % 2228
  \author[\instIITGuwahati]{B.~Bhuyan,} % 2097
  \author[\instTorinoUNIV,\instTorinoINFN]{F.~Bianchi,} % 2564
  \author[\instPrague]{T.~Bilka,} % 2484
% \author[\instLMU]{S.~Bilokin,} % 3623
  \author[\instLouisville]{D.~Biswas,} % 8703
  \author[\instBINP,\instNSU]{A.~Bobrov,} % 2294
  \author[\instSoochow,\instHSE]{D.~Bodrov,} % 9643
  \author[\instDESY]{A.~Bolz,} % 15403
  \author[\instBINP,\instNSU]{A.~Bondar,} % 4643
% \author[\instWayneState]{G.~Bonvicini,} % 2095
% \author[\instIITGuwahati]{J.~Borah,} % 7083
  \author[\instKrakow]{A.~Bozek,} % 2303
  \author[\instLjubljanaJSI,\instLjubljanaUM]{M.~Bra\v{c}ko,} % 2425
  \author[\instRomaTreINFN]{P.~Branchini,} % 2577
% \author[\instCMU]{R.~A.~Briere,} % 2584
  \author[\instHawaii]{T.~E.~Browder,} % 2560
  \author[\instRomaTreINFN]{A.~Budano,} % 2171
  \author[\instRomaTreUNIV,\instRomaTreINFN]{S.~Bussino,} % 5384
% \author[\instFrascati]{A.~Calcaterra,} % 19163
  \author[\instNapoliINFN]{M.~Campajola,} % 5223
  \author[\instDESY]{L.~Cao,} % 2099
  \author[\instPisaUNIV,\instPisaINFN]{G.~Casarosa,} % 2491
  \author[\instPerugiaUNIV,\instPerugiaINFN]{C.~Cecchi,} % 2433
  \author[\instIPHC]{J.~Cerasoli,} % 20746
  \author[\instFuJen]{M.-C.~Chang,} % 2827
  \author[\instNTUTaiwan]{P.~Chang,} % 2542
% \author[\instDESY]{R.~Cheaib,} % 2208
  \author[\instSydney]{P.~Cheema,} % 15264
% \author[\instMPP]{V.~Chekelian,} % 2167
% \author[\instISU]{C.~Chen,} % 12803
% \author[\instJLU]{Y.~Q.~Chen,} % 16264
% \author[\instNTUTaiwan]{Y.-T.~Chen,} % 2884
  \author[\instHanyang]{B.~G.~Cheon,} % 2173
  \author[\instBINP]{K.~Chilikin,} % 2308
  \author[\instChiangMai]{K.~Chirapatpimol,} % 10803
  \author[\instHanyang]{H.-E.~Cho,} % 2182
  \author[\instKISTI]{K.~Cho,} % 2516
  \author[\instYonsei]{S.-J.~Cho,} % 2723
  \author[\instCAU]{S.-K.~Choi,} % 2364
  \author[\instISU]{S.~Choudhury,} % 2206
% \author[\instWayneState]{D.~Cinabro,} % 2092
% \author[\instISU]{J.~Cochran,} % 12604
  \author[\instPisaUNIV,\instPisaINFN]{L.~Corona,} % 3944
% \author[\instMississippi]{L.~M.~Cremaldi,} % 2276
% \author[\instDESY]{S.~Cunliffe,} % 2272
% \author[\instTokyoMetropolitan]{T.~Czank,} % 2254
  \author[\instMNITJaipur]{S.~Das,} % 9163
  \author[\instDESY]{F.~Dattola,} % 3745
  \author[\instCinvestavIPN]{E.~De~La~Cruz-Burelo,} % 2359
  \author[\instAdelaide]{S.~A.~De~La~Motte,} % 2128
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{G.~de~Marino,} % 8364
  \author[\instNapoliUNIV,\instNapoliINFN]{G.~De~Nardo,} % 2459
  \author[\instUBC]{M.~De~Nuccio,} % 2610
  \author[\instKarlsruhe]{G.~De~Pietro,} % 2528
  \author[\instFrascati]{R.~de~Sangro,} % 2524
% \author[\instBonn]{B.~Deschamps,} % 2671
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Destefanis,} % 2594
% \author[\instTelAviv]{S.~Dey,} % 5023
% \author[\instCinvestavIPN]{A.~De~Yta-Hernandez,} % 2104
  \author[\instIITHyderabad]{R.~Dhamija,} % 9465
  \author[\instBNL]{A.~Di~Canto,} % 10963
  \author[\instNapoliUNIV,\instNapoliINFN]{F.~Di~Capua,} % 2065
  \author[\instBonn]{J.~Dingfelder,} % 2151
  \author[\instPrague]{Z.~Dole\v{z}al,} % 2319
% \author[\instUAS]{I.~Dom\'{\i}nguez~Jim\'{e}nez,} % 2191
  \author[\instITAR]{T.~V.~Dong,} % 2215
  \author[\instTriesteINFN]{M.~Dorigo,} % 12543
% \author[\instHEPHYVienna]{D.~Dorner,} % 13564
  \author[\instGiessen]{K.~Dort,} % 5583
% \author[\instMelbourne]{D.~Dossett,} % 2574
  \author[\instDESY]{S.~Dreyer,} % 12823
  \author[\instHawaii]{S.~Dubey,} % 11063
% \author[\instBonn]{S.~Duell,} % 2344
  \author[\instIPHC]{G.~Dujany,} % 9703
  \author[\instKarlsruhe]{P.~Ecker,} % 5563
  \author[\instBonn]{M.~Eliachevitch,} % 2725
% \author[\instBINP,\instNSU]{D.~Epifanov,} % 2551
  \author[\instHEPHYVienna]{P.~Feichtinger,} % 9843
  \author[\instKarlsruhe]{T.~Ferber,} % 2482
  \author[\instMelbourne]{D.~Ferlewicz,} % 2073
  \author[\instKEK]{T.~Fillinger,} % 9803
  \author[\instIPHC]{C.~Finck,} % 15803
  \author[\instFrascati]{G.~Finocchiaro,} % 2400
% \author[\instHeidelberg]{P.~Fischer,} % 2141
% \author[\instHawaii]{K.~Flood,} % 12103
  \author[\instMcGill]{A.~Fodor,} % 2312
  \author[\instPisaUNIV,\instPisaINFN]{F.~Forti,} % 2432
  \author[\instGoettingen]{A.~Frey,} % 2150
% \author[\instHEPHYVienna]{M.~Friedl,} % 2442
  \author[\instPNNL]{B.~G.~Fulsom,} % 2563
  \author[\instTriesteUNIV,\instTriesteINFN]{A.~Gabrielli,} % 13523
% \author[\instBINP,\instNSU]{N.~Gabyshev,} % 2510
  \author[\instDESY]{E.~Ganiev,} % 4623
  \author[\instKEK]{M.~Garcia-Hernandez,} % 4823
  \author[\instCMU]{R.~Garg,} % 2213
% \author[\instBINP,\instNSU]{A.~Garmash,} % 2161
  \author[\instNapoliINFN]{G.~Gaudino,} % 16563
  \author[\instUPES]{V.~Gaur,} % 2413
  \author[\instPadovaUNIV,\instPadovaINFN]{A.~Gaz,} % 2181
% \author[\instGoettingen]{U.~Gebauer,} % 2174
  \author[\instDESY]{A.~Gellrich,} % 2480
  \author[\instYerevan]{G.~Ghevondyan,} % 9445
  \author[\instTriesteUNIV,\instTriesteINFN]{D.~Ghosh,} % 11923
  \author[\instYerevan]{H.~Ghumaryan,} % 19543
  \author[\instBonn]{G.~Giakoustidis,} % 13723
  \author[\instNapoliUNIV,\instNapoliINFN]{R.~Giordano,} % 2103
  \author[\instIITHyderabad]{A.~Giri,} % 2106
% \author[\instDESY]{A.~Glazov,} % 2473
  \author[\instTriesteINFN]{B.~Gobbo,} % 2109
  \author[\instSAlabama]{R.~Godang,} % 2449
  \author[\instKyiv]{O.~Gogota,} % 2334
  \author[\instKarlsruhe]{P.~Goldenzweig,} % 2345
% \author[\instLjubljanaUniLJ,\instNovaGorica,\instLjubljanaJSI]{B.~Golob,} % 3703
% \author[\instUSTC]{G.~Gong,} % 2727
% \author[\instAdelaide]{P.~Grace,} % 9563
  \author[\instMainz]{W.~Gradl,} % 2570
% \author[\instDESY]{M.~Graf-Schreiber,} % 2730
  \author[\instVictoria]{T.~Grammatico,} % 20623
% \author[\instBonn]{S.~Granderath,} % 8383
  \author[\instRomaTreINFN]{E.~Graziani,} % 2342
  \author[\instTUM]{D.~Greenwald,} % 2686
  \author[\instPrague]{Z.~Gruberov\'{a},} % 8824
  \author[\instPittsburgh]{T.~Gu,} % 14283
  \author[\instCincinnati]{Y.~Guan,} % 2514
  \author[\instBINP,\instNSU]{K.~Gudkova,} % 10504
% \author[\instHEPHYVienna]{H.~Haigh,} % 16744
  \author[\instTata]{S.~Halder,} % 4743
  \author[\instDESY]{Y.~Han,} % 19663
% \author[\instKEK,\instSOKENDAI]{K.~Hara,} % 2462
  \author[\instKEK,\instSOKENDAI]{T.~Hara,} % 2523
% \author[\instHawaii]{O.~Hartbrich,} % 2158
% \author[\instNiigata]{K.~Hayasaka,} % 2330
  \author[\instNaraWu]{H.~Hayashii,} % 2455
  \author[\instTata]{S.~Hazra,} % 7663
  \author[\instUBC,\instIPP]{C.~Hearty,} % 2450
  \author[\instBonn]{M.~T.~Hedges,} % 2265
  \author[\instKarlsruhe]{A.~Heidelbach,} % 16923
  \author[\instCinvestavIPN,\instConacyt]{I.~Heredia~de~la~Cruz,} % 2559
  \author[\instDESY]{M.~Hern\'{a}ndez~Villanueva,} % 2466
% \author[\instUBC]{A.~Hershenhorn,} % 2552
  \author[\instIPMU]{T.~Higuchi,} % 2485
% \author[\instNagoya]{H.~Hirata,} % 2070
  \author[\instMainz]{M.~Hoek,} % 2101
  \author[\instMelbourne]{M.~Hohmann,} % 2077
  \author[\instHEPHYVienna]{P.~Horak,} % 13583
% \author[\instRCNP]{T.~Hotta,} % 2084
  \author[\instSydney]{C.-L.~Hsu,} % 2299
% \author[\instNTUTaiwan]{K.~Huang,} % 2389
  \author[\instDESY]{T.~Humair,} % 10643
  \author[\instNagoya,\instNagoyaKMI,\instKEK]{T.~Iijima,} % 2446
% \author[\instNagoya,\instKEK]{K.~Inami,} % 2323
% \author[\instHEPHYVienna]{G.~Inguglia,} % 2500
  \author[\instIITHyderabad]{N.~Ipsita,} % 12223
% \author[\instKarlsruhe]{J.~Irakkathil~Jabbar,} % 7343
  \author[\instKEK,\instSOKENDAI]{A.~Ishikawa,} % 2281
% \author[\instKEK]{S.~Ito,} % 17463
  \author[\instKEK,\instSOKENDAI]{R.~Itoh,} % 2487
  \author[\instOsakaMetropolitan]{M.~Iwasaki,} % 2360
% \author[\instKEK]{Y.~Iwasaki,} % 2229
% \author[\instTokyoMetropolitan]{S.~Iwata,} % 4323
  \author[\instAdelaide]{P.~Jackson,} % 2255
  \author[\instIndiana]{W.~W.~Jacobs,} % 2322
% \author[\instBNL]{D.~E.~Jaffe,} % 3663
  \author[\instGyeongsang]{E.-J.~Jang,} % 6744
  \author[\instHNU]{Q.~P.~Ji,} % 16243
  \author[\instSEU]{S.~Jia,} % 2457
  \author[\instBNL]{Y.~Jin,} % 2105
% \author[\instIITMadras]{A.~Johnson,} % 16143
  \author[\instChonnam]{K.~K.~Joo,} % 4224
  \author[\instBonn]{H.~Junkerkalefeld,} % 12963
% \author[\instKyiv]{I.~Kadenko,} % 3843
  \author[\instTokyoMetropolitan]{H.~Kakuno,} % 2391
% \author[\instKrakow]{M.~Kaleta,} % 5603
  \author[\instIITGuwahati]{D.~Kalita,} % 2220
  \author[\instHEPHYVienna]{A.~B.~Kaliyar,} % 7344
  \author[\instPadovaINFN]{J.~Kandra,} % 2541
  \author[\instIPMU]{K.~H.~Kang,} % 2283
  \author[\instISU]{S.~Kang,} % 12683
% \author[\instKrakow]{P.~Kapusta,} % 6663
  \author[\instYerevan]{G.~Karyan,} % 2550
% \author[\instNagoya,\instNagoyaKMI]{Y.~Kato,} % 2549
% \author[\instChiba]{H.~Kawai,} % 4344
  \author[\instKitasato]{T.~Kawasaki,} % 4363
  \author[\instMainz]{F.~Keil,} % 19523
% \author[\instHawaii]{C.~Ketter,} % 2236
  \author[\instMPP]{C.~Kiesling,} % 2168
  \author[\instHanyang]{C.-H.~Kim,} % 2358
  \author[\instSoongsil]{D.~Y.~Kim,} % 2315
% \author[\instKyungpook]{H.~J.~Kim,} % 4863
  \author[\instKISTI]{K.-H.~Kim,} % 2118
% \author[\instKoreaUnivKU]{K.~Kim,} % 2409
  \author[\instYonsei]{Y.-K.~Kim,} % 2379
% \author[\instKoreaUnivKU]{Y.~J.~Kim,} % 2403
% \author[\instVPI]{T.~D.~Kimmel,} % 2241
  \author[\instVPI,\instKEK]{H.~Kindo,} % 2195
  \author[\instCincinnati]{K.~Kinoshita,} % 2318
% \author[\instDESY]{C.~Kleinwort,} % 2499
  \author[\instPrague]{P.~Kody\v{s},} % 2407
  \author[\instKEK]{T.~Koga,} % 6963
  \author[\instHawaii]{S.~Kohani,} % 9143
  \author[\instNagoya]{K.~Kojima,} % 6363
% \author[\instKitasato]{T.~Konno,} % 2490
  \author[\instBINP,\instNSU]{A.~Korobov,} % 4185
  \author[\instLjubljanaJSI,\instLjubljanaUM]{S.~Korpar,} % 2475
% \author[\instIJCLab]{E.~Kou,} % 3765
  \author[\instBINP,\instNSU]{E.~Kovalenko,} % 3884
  \author[\instVictoria]{R.~Kowalewski,} % 2293
  \author[\instMPP]{T.~M.~G.~Kraetzschmar,} % 7543
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{P.~Kri\v{z}an,} % 2474
% \author[\instMississippi]{R.~Kroeger,} % 2242
% \author[\instMelbourne]{J.~F.~Krohn,} % 2502
  \author[\instBINP,\instNSU]{P.~Krokovny,} % 2575
% \author[\instGiessen]{W.~Kuehn,} % 2534
% \author[\instDESY,\instLMU]{M.~K\"{u}nzel,} % 2139
  \author[\instLMU]{T.~Kuhr,} % 2486
% \author[\instLMU]{Y.~Kulii,} % 9823
% \author[\instIITJodhpur]{J.~Kumar,} % 6464
  \author[\instIISER]{M.~Kumar,} % 2744
% \author[\instPanjabPAU]{R.~Kumar,} % 2189
  \author[\instMississippi]{K.~Kumara,} % 2257
% \author[\instTokyoMetropolitan]{T.~Kumita,} % 4083
  \author[\instKEK]{T.~Kunigo,} % 10104
% \author[\instNaraWu]{A.~Kusudo,} % 14623
  \author[\instBINP,\instNSU]{A.~Kuzmin,} % 2520
% \author[\instPrague]{P.~Kvasni\v{c}ka,} % 2184
  \author[\instYonsei]{Y.-J.~Kwon,} % 2231
  \author[\instPadovaINFN]{S.~Lacaprara,} % 2447
  \author[\instKEK]{Y.-T.~Lai,} % 2066
% \author[\instIPMU]{C.~La~Licata,} % 2348
% \author[\instMNITJaipur]{K.~Lalwani,} % 2142
  \author[\instVPI]{T.~Lam,} % 2729
  \author[\instTriesteINFN]{L.~Lanceri,} % 2540
  \author[\instGiessen]{J.~S.~Lange,} % 2277
  \author[\instUppsala]{M.~Laurenza,} % 10223
% \author[\instCPPM]{K.~Lautenbach,} % 2102
% \author[\instBNL]{P.~J.~Laycock,} % 7683
  \author[\instCPPM]{R.~Leboucher,} % 14083
  \author[\instIJCLab]{F.~R.~Le~Diberder,} % 3267
  \author[\instSKKU]{M.~J.~Lee,} % 21803
% \author[\instKyungpook]{S.~C.~Lee,} % 2544
% \author[\instMPP]{P.~Leitl,} % 2414
% \author[\instCPPM]{C.~Lemettais,} % 22704
  \author[\instKEK]{D.~Levit,} % 2507
% \author[\instBonn]{P.~M.~Lewis,} % 2582
  \author[\instLNNU]{C.~Li,} % 2325
  \author[\instCincinnati]{L.~K.~Li,} % 3263
% \author[\instFudan]{S.~X.~Li,} % 2377
  \author[\instFudan]{Y.~Li,} % 8083
  \author[\instFudan]{Y.~B.~Li,} % 2573
  \author[\instIITMadras]{J.~Libby,} % 2262
% \author[\instLMU]{K.~Lieret,} % 2268
% \author[\instNTUTaiwan]{J.~Lin,} % 2401
% \author[\instNTUTaiwan]{Y.-R.~Lin,} % 9323
% \author[\instHiroshima]{Z.~Liptak,} % 3565
  \author[\instFudan]{M.~Liu,} % 15244
  \author[\instDESY]{Q.~Y.~Liu,} % 7045
% \author[\instIHEPChina]{Z.~A.~Liu,} % 3283
  \author[\instShandong]{Z.~Q.~Liu,} % 11303
  \author[\instWayneState,\instKEK]{D.~Liventsev,} % 2578
  \author[\instManitoba]{S.~Longo,} % 2396
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Lozar,} % 12423
  \author[\instLMU]{T.~Lueck,} % 2406
% \author[\instFudan]{T.~Luo,} % 3268
  \author[\instBonn]{C.~Lyu,} % 12484
  \author[\instRIKENMSL]{Y.~Ma,} % 16883
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Maggiora,} % 5343
  \author[\instIITHyderabad]{S.~P.~Maharana,} % 19083
  \author[\instHEPHYVienna]{R.~Maiti,} % 12043
  \author[\instIITBhubaneswar]{S.~Maity,} % 2985
  \author[\instCPPM]{G.~Mancinelli,} % 20743
  \author[\instTriesteUNIV,\instTriesteINFN]{R.~Manfredi,} % 10303
  \author[\instPerugiaINFN]{E.~Manoni,} % 2305
% \author[\instBonn]{A.~C.~Manthei,} % 15023
  \author[\instTriesteUNIV,\instTriesteINFN]{M.~Mantovano,} % 19783
  \author[\instMelbourne]{D.~Marcantonio,} % 11163
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Marcello,} % 4223
  \author[\instIFIC]{C.~Marinas,} % 2133
  \author[\instIPHC]{L.~Martel,} % 13503
  \author[\instRomaTreINFN]{C.~Martellini,} % 16983
  \author[\instDESY]{A.~Martini,} % 2336
  \author[\instDESY]{T.~Martinov,} % 19463
  \author[\instPisaUNIV,\instPisaINFN]{L.~Massaccesi,} % 16323
  \author[\instRCNP,\instEri]{M.~Masuda,} % 2238
% \author[\instUOM]{T.~Matsuda,} % 5543
  \author[\instKEK,\instNagoya]{K.~Matsuoka,} % 2316
  \author[\instBINP,\instNSU]{D.~Matvienko,} % 2351
  \author[\instIITGuwahati]{S.~K.~Maurya,} % 9763
  \author[\instUBC]{J.~A.~McKenna,} % 2392
% \author[\instMPP]{F.~Meggendorfer,} % 7103
  \author[\instTata]{R.~Mehta,} % 15203
  \author[\instDuke]{F.~Meier,} % 3103
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Merola,} % 2456
  \author[\instBonn]{F.~Metzner,} % 2296
% \author[\instMelbourne]{M.~Milesi,} % 5443
  \author[\instVictoria]{C.~Miller,} % 2273
  \author[\instNapoliINFN]{M.~Mirra,} % 14744
  \author[\instNaraWu,\instKEK]{K.~Miyabayashi,} % 2327
  \author[\instKEK,\instSOKENDAI]{H.~Miyake,} % 2452
  \author[\instIJCLab]{R.~Mizuk,} % 2483
  \author[\instTata]{G.~B.~Mohanty,} % 2278
  \author[\instCinvestavIPN]{N.~Molina-Gonzalez,} % 8004
  \author[\instPisaUNIV,\instPisaINFN]{S.~Mondal,} % 19743
  \author[\instPerugiaUNIV,\instPerugiaINFN]{S.~Moneta,} % 13303
% \author[\instKoreaUnivKU]{H.~Moon,} % 2304
  \author[\instMPP]{H.-G.~Moser,} % 2120
  \author[\instHEPHYVienna]{M.~Mrvar,} % 2527
% \author[\instKarlsruhe]{Th.~Muller,} % 2165
  \author[\instTorinoINFN]{R.~Mussa,} % 2372
  \author[\instKEK,\instSOKENDAI]{I.~Nakamura,} % 3463
% \author[\instKEK,\instSOKENDAI]{K.~R.~Nakamura,} % 2417
% \author[\instOsakaMetropolitan]{E.~Nakano,} % 2554
% \author[\instKEK,\instSOKENDAI]{M.~Nakao,} % 2498
% \author[\instKEK,\instSOKENDAI]{H.~Nakayama,} % 2232
% \author[\instNTUTaiwan]{H.~Nakazawa,} % 2335
  \author[\instKEK]{Y.~Nakazawa,} % 17383
  \author[\instDESY]{A.~Narimani~Charan,} % 10143
  \author[\instKyotoU]{M.~Naruki,} % 4583
  \author[\instIITGuwahati]{D.~Narwal,} % 7223
  \author[\instKrakow]{Z.~Natkaniec,} % 3923
  \author[\instHawaii]{A.~Natochii,} % 12063
  \author[\instIITHyderabad]{L.~Nayak,} % 9464
  \author[\instTelAviv]{M.~Nayak,} % 2371
  \author[\instYerevan]{G.~Nazaryan,} % 9523
  \author[\instDESY]{C.~Niebuhr,} % 2477
% \author[\instKSU]{M.~Niiyama,} % 2063
% \author[\instMPGHLL]{J.~Ninkovic,} % 2386
% \author[\instBNL]{N.~K.~Nisar,} % 2522
  \author[\instKEK,\instSOKENDAI,\instNiigata]{S.~Nishida,} % 2571
% \author[\instHawaii]{K.~Nishimura,} % 3063
% \author[\instMalaya]{M.~H.~A.~Nouxman,} % 2470
% \author[\instNiigata]{K.~Ogawa,} % 2430
  \author[\instToho]{S.~Ogawa,} % 6263
% \author[\instCAU]{S.~L.~Olsen,} % 4563
  \author[\instKyiv]{Y.~Onishchuk,} % 2157
  \author[\instNiigata]{H.~Ono,} % 2160
  \author[\instUTokyo]{Y.~Onuki,} % 2331
  \author[\instIJCLab]{P.~Oskin,} % 9623
  \author[\instUTokyo]{F.~Otani,} % 16244
% \author[\instCMU]{E.~R.~Oxford,} % 6943
% \author[\instKEK,\instSOKENDAI]{H.~Ozaki,} % 2984
  \author[\instHSE]{P.~Pakhlov,} % 2221
  \author[\instHSE]{G.~Pakhlova,} % 2188
% \author[\instPisaUNIV,\instPisaINFN]{A.~Paladino,} % 2435
% \author[\instPittsburgh]{T.~Pang,} % 2114
  \author[\instMississippi]{A.~Panta,} % 7943
% \author[\instPisaUNIV,\instPisaINFN]{E.~Paoloni,} % 2488
  \author[\instNapoliINFN]{S.~Pardi,} % 2532
  \author[\instDuke]{K.~Parham,} % 10684
  \author[\instKyungpook]{H.~Park,} % 2284
  \author[\instKEK]{S.-H.~Park,} % 2509
  \author[\instBonn]{B.~Paschen,} % 2159
  \author[\instRomaTreINFN]{A.~Passeri,} % 2116
  \author[\instLouisville]{S.~Patra,} % 3123
  \author[\instTUM]{S.~Paul,} % 2131
  \author[\instLuther]{T.~K.~Pedlar,} % 2421
% \author[\instFrascati]{I.~Peruzzi,} % 2253
  \author[\instHawaii]{R.~Peschke,} % 7123
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{R.~Pestotnik,} % 2476
% \author[\instMelbourne]{F.~Pham,} % 2963
  \author[\instFrascati]{M.~Piccolo,} % 2147
  \author[\instVPI]{L.~E.~Piilonen,} % 2346
  \author[\instTorinoUNIV,\instTorinoINFN]{G.~Pinna~Angioni,} % 13363
  \author[\instUAS]{P.~L.~M.~Podesta-Lerma,} % 2266
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{T.~Podobnik,} % 11223
  \author[\instMississippi]{S.~Pokharel,} % 12283
% \author[\instCPPM]{L.~Polat,} % 9783
% \author[\instTelAviv,\instHSE]{V.~Popov,} % 2096
  \author[\instKEK]{C.~Praz,} % 2726
  \author[\instISU]{S.~Prell,} % 12743
  \author[\instGiessen]{E.~Prencipe,} % 2219
  \author[\instBonn]{M.~T.~Prim,} % 2501
% \author[\instOkinawa]{M.~V.~Purohit,} % 2196
  \author[\instHawaii]{H.~Purwar,} % 12363
% \author[\instDESY]{N.~Rad,} % 11683
  \author[\instHEPHYVienna]{P.~Rados,} % 7383
  \author[\instHEPHYVienna]{G.~Raeuber,} % 18143
  \author[\instTriesteUNIV,\instTriesteINFN]{S.~Raiz,} % 13003
% \author[\instKyungpook]{A.~Ramirez~Morales,} % 13724
  \author[\instGoettingen]{N.~Rauls,} % 11603
  \author[\instMPP]{M.~Reif,} % 8043
  \author[\instGiessen]{S.~Reiter,} % 2248
  \author[\instBINP,\instNSU]{M.~Remnev,} % 2785
  \author[\instIPHC]{I.~Ripp-Baudot,} % 2469
% \author[\instHeidelberg]{M.~Ritzert,} % 2526
  \author[\instPisaUNIV,\instPisaINFN]{G.~Rizzo,} % 2579
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~B.~Rizzuto,} % 3746
  \author[\instMcGill,\instIPP]{S.~H.~Robertson,} % 2471
% \author[\instMelbourne]{P.~Rocchetti,} % 13763
% \author[\instUAS]{D.~Rodr\'{i}guez~P\'{e}rez,} % 2176
  \author[\instDESY]{M.~Roehrken,} % 11883
  \author[\instVictoria,\instIPP]{J.~M.~Roney,} % 2244
% \author[\instSCarolina]{C.~Rosenfeld,} % 2082
  \author[\instDESY]{A.~Rostomyan,} % 2481
  \author[\instTriesteINFN]{N.~Rout,} % 2965
% \author[\instKrakow]{M.~Rozanska,} % 2205
  \author[\instNapoliUNIV,\instNapoliINFN]{G.~Russo,} % 2388
% \author[\instISU]{D.~Sahoo,} % 2110
% \author[\instKEK,\instSOKENDAI]{Y.~Sakai,} % 2175
  \author[\instMississippi]{D.~A.~Sanders,} % 2458
  \author[\instIITHyderabad]{S.~Sandilya,} % 2286
% \author[\instCincinnati]{A.~Sangal,} % 2384
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~Santelj,} % 2185
% \author[\instPadovaUNIV,\instPadovaINFN]{P.~Sartori,} % 4523
  \author[\instKEK]{Y.~Sato,} % 5243
  \author[\instPittsburgh]{V.~Savinov,} % 2292
  \author[\instUppsala]{B.~Scavino,} % 2518
% \author[\instLMU,\instMPP]{C.~Schmitt,} % 15063
% \author[\instBonn]{J.~Schmitz,} % 12863
% \author[\instKarlsruhe]{M.~Schnepf,} % 15683
% \author[\instHawaii]{J.~Schueler,} % 2824
  \author[\instHEPHYVienna]{C.~Schwanda,} % 2108
% \author[\instCincinnati]{A.~J.~Schwartz,} % 2162
% \author[\instGoettingen]{B.~Schwenker,} % 2405
% \author[\instGoettingen]{M.~Schwickardi,} % 14743
  \author[\instNiigata]{Y.~Seino,} % 2517
  \author[\instRomaTreINFN]{A.~Selce,} % 9043
  \author[\instYamagata]{K.~Senyo,} % 2987
  \author[\instCPPM]{J.~Serrano,} % 12124
  \author[\instMelbourne]{M.~E.~Sevior,} % 2328
  \author[\instMainz]{C.~Sfienti,} % 2214
  \author[\instHUNNU]{W.~Shan,} % 11943
% \author[\instMNITJaipur]{C.~Sharma,} % 11584
% \author[\instHawaii]{V.~Shebalin,} % 2339
  \author[\instFudan]{C.~P.~Shen,} % 2464
  \author[\instKEK]{X.~D.~Shi,} % 18843
% \author[\instToho]{H.~Shibuya,} % 2234
  \author[\instMcGill]{T.~Shillington,} % 7983
  \author[\instUTokyo]{T.~Shimasaki,} % 16263
  \author[\instNTUTaiwan]{J.-G.~Shiu,} % 2412
  \author[\instBINP,\instNSU]{D.~Shtol,} % 9223
  \author[\instBINP,\instNSU]{B.~Shwartz,} % 2122
  \author[\instHawaii]{A.~Sibidanov,} % 2419
  \author[\instKarlsruhe]{F.~Simon,} % 2164
  \author[\instPanjab]{J.~B.~Singh,} % 2903
  \author[\instMPP]{J.~Skorupa,} % 12523
% \author[\instMelbourne]{K.~Smith,} % 2243
  \author[\instVictoria,\instIPP]{R.~J.~Sobie,} % 2472
  \author[\instMainz]{M.~Sobotzik,} % 8604
  \author[\instTelAviv]{A.~Soffer,} % 2217
  \author[\instIHEPRussia]{A.~Sokolov,} % 2521
% \author[\instDESY]{Y.~Soloviev,} % 2479
  \author[\instBINP]{E.~Solovieva,} % 2398
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Spataro,} % 2117
  \author[\instMainz]{B.~Spruck,} % 2493
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{M.~Stari\v{c},} % 2326
  \author[\instIPHC]{P.~Stavroulakis,} % 20643
  \author[\instKarlsruhe]{S.~Stefkova,} % 8783
% \author[\instVPI]{Z.~S.~Stottler,} % 2267
  \author[\instPadovaUNIV,\instPadovaINFN]{R.~Stroili,} % 2465
% \author[\instPNNL]{J.~Strube,} % 2451
% \author[\instKrakow]{J.~Stypula,} % 2368
% \author[\instNagoya]{Y.~Sue,} % 2085
% \author[\instUTokyo]{R.~Sugiura,} % 4644
  \author[\instRCNP,\instGifu]{M.~Sumihama,} % 4243
  \author[\instKEK,\instSOKENDAI,\instNaraWu]{K.~Sumisawa,} % 2583
  \author[\instBonn]{W.~Sutcliffe,} % 3784
% \author[\instKEK,\instSOKENDAI]{S.~Y.~Suzuki,} % 2496
  \author[\instDESY]{H.~Svidras,} % 11783
% \author[\instChiba]{M.~Tabata,} % 2986
% \author[\instDESY]{M.~Takahashi,} % 2467
  \author[\instSPU,\instJPARC,\instRIKENMSL]{M.~Takizawa,} % 2437
  \author[\instTorinoINFN]{U.~Tamponi,} % 2366
% \author[\instKEK,\instSOKENDAI]{S.~Tanaka,} % 2530
  \author[\instJAEA]{K.~Tanida,} % 3803
% \author[\instUTokyo]{H.~Tanigawa,} % 2237
% \author[\instKEK]{N.~Taniguchi,} % 2285
  \author[\instPisaUNIV,\instPisaINFN]{F.~Tenchini,} % 2546
% \author[\instCPPM]{A.~Thaller,} % 16044
  \author[\instMPP]{O.~Tittel,} % 8663
  \author[\instTata]{R.~Tiwary,} % 10403
  \author[\instTriesteINFN]{D.~Tonelli,} % 4564
  \author[\instPadovaINFN]{E.~Torassa,} % 2556
% \author[\instSydney]{N.~Toutounji,} % 2263
  \author[\instIJCLab]{K.~Trabelsi,} % 2369
  \author[\instBonn]{I.~Tsaklidis,} % 13443
% \author[\instKEK,\instSOKENDAI]{T.~Tsuboyama,} % 2361
% \author[\instNagoya]{N.~Tsuzuki,} % 2352
  \author[\instTitech]{M.~Uchida,} % 2370
  \author[\instKEK,\instSOKENDAI]{I.~Ueda,} % 2519
% \author[\instKEK,\instSOKENDAI]{S.~Uehara,} % 2586
% \author[\instUTokyo]{Y.~Uematsu,} % 5883
  \author[\instHSE]{T.~Uglov,} % 2252
  \author[\instKarlsruhe]{K.~Unger,} % 9463
  \author[\instHanyang]{Y.~Unno,} % 2420
  \author[\instKEK]{K.~Uno,} % 14963
  \author[\instKEK,\instSOKENDAI]{S.~Uno,} % 2149
  \author[\instMelbourne]{P.~Urquijo,} % 2302
  \author[\instKEK,\instUTokyo,\instSOKENDAI]{Y.~Ushiroda,} % 2317
% \author[\instBINP,\instNSU]{Y.~V.~Usov,} % 5003
  \author[\instHawaii]{S.~E.~Vahsen,} % 2251
  \author[\instMcGill]{R.~van~Tonder,} % 2706
% \author[\instHawaii]{G.~S.~Varner,} % 2119
  \author[\instSydney]{K.~E.~Varvell,} % 2545
  \author[\instISU]{M.~Veronesi,} % 20723
  \author[\instBINP,\instNSU]{A.~Vinokurova,} % 2289
  \author[\instIITHyderabad]{V.~S.~Vismaya,} % 16063
  \author[\instTriesteUNIV,\instTriesteINFN]{L.~Vitale,} % 2415
  \author[\instIJCLab]{V.~Vobbilisetti,} % 7364
  \author[\instPerugiaUNIV,\instPerugiaINFN]{R.~Volpe,} % 20183
% \author[\instBINP]{V.~Vorobyev,} % 2298
% \author[\instDuke]{A.~Vossen,} % 2249
  \author[\instMPP]{B.~Wach,} % 8203
% \author[\instKEK]{E.~Waheed,} % 2226
  \author[\instUBC]{M.~Wakai,} % 3583
% \author[\instMcGill]{H.~M.~Wakeling,} % 3664
  \author[\instMPP]{S.~Wallner,} % 20363
% \author[\instMalaya]{W.~Wan~Abdullah,} % 2280
% \author[\instMPP]{B.~Wang,} % 2569
% \author[\instNUUTaiwan]{C.~H.~Wang,} % 2224
  \author[\instPittsburgh]{E.~Wang,} % 10983
  \author[\instNTUTaiwan]{M.-Z.~Wang,} % 2074
  \author[\instFudan]{X.~L.~Wang,} % 2076
  \author[\instUTokyo]{Z.~Wang,} % 15743
  \author[\instMcGill]{A.~Warburton,} % 2347
% \author[\instNiigata]{M.~Watanabe,} % 2309
  \author[\instYonsei]{S.~Watanuki,} % 6843
% \author[\instBonn]{M.~Welsch,} % 7023
% \author[\instTriesteINFN]{O.~Werbycka,} % 6123
  \author[\instDESY]{C.~Wessel,} % 2100
% \author[\instKrakow]{J.~Wiechczynski,} % 2604
% \author[\instGoettingen]{P.~Wieduwilt,} % 2343
% \author[\instMPP]{H.~Windel,} % 2081
  \author[\instKoreaUnivKU]{E.~Won,} % 2410
% \author[\instShandong]{Y.~Xie,} % 20383
  \author[\instSoochow]{X.~P.~Xu,} % 4923
  \author[\instSydney]{B.~D.~Yabsley,} % 3645
  \author[\instKEK]{S.~Yamada,} % 2492
% \author[\instUSTC]{W.~Yan,} % 2094
  \author[\instKoreaUnivKU]{S.~B.~Yang,} % 2374
  \author[\instFlorida]{J.~Yelton,} % 2067
  \author[\instKoreaUnivKU]{J.~H.~Yin,} % 2365
% \author[\instIHEPChina]{Y.~M.~Yook,} % 2453
  \author[\instNagoya]{K.~Yoshihara,} % 12663
  \author[\instIHEPChina]{C.~Z.~Yuan,} % 2088
  \author[\instNiigata]{Y.~Yusa,} % 2357
  \author[\instRomaTreUNIV,\instRomaTreINFN]{L.~Zani,} % 2529
  \author[\instHawaii]{B.~Zhang,} % 11663
% \author[\instIHEPChina]{J.~Z.~Zhang,} % 2349
  \author[\instFudan]{Y.~Zhang,} % 3303
% \author[\instUSTC]{Z.~Zhang,} % 5363
  \author[\instBINP,\instNSU]{V.~Zhilich,} % 4703
% \author[\instFudan]{J.~S.~Zhou,} % 12463
  \author[\instShandong]{Q.~D.~Zhou,} % 7323
  \author[\instLNNU]{X.~Y.~Zhou,} % 2380
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{V.~I.~Zhukova,} % 2387
% \author[\instBINP,\instNSU]{V.~Zhulanov,} % 4983
% \author[\instPrague]{R.~\v{Z}leb\v{c}\'{i}k} % 13403
%%%\affiliation[\instSinica]{Academia Sinica, Taipei 11529, Taiwan}
\affiliation[\instCPPM]{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\affiliation[\instYerevan]{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\affiliation[\instGoettingen]{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
%%%\affiliation[\instBeihang]{Beihang University, Beijing 100191, China}
\affiliation[\instBNL]{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\affiliation[\instBINP]{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\affiliation[\instCMU]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\affiliation[\instCinvestavIPN]{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\affiliation[\instPrague]{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\affiliation[\instChiangMai]{Chiang Mai University, Chiang Mai 50202, Thailand}
%%%\affiliation[\instChiba]{Chiba University, Chiba 263-8522, Japan}
\affiliation[\instChonnam]{Chonnam National University, Gwangju 61186, South Korea}
%%%\affiliation[\instChula]{Chulalongkorn University, Bangkok 10330, Thailand}
\affiliation[\instCAU]{Chung-Ang University, Seoul 06974, South Korea}
\affiliation[\instConacyt]{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\affiliation[\instDESY]{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\affiliation[\instDuke]{Duke University, Durham, North Carolina 27708, U.S.A.}
\affiliation[\instITAR]{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
%%%\affiliation[\instJuelich]{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\affiliation[\instFuJen]{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\affiliation[\instFudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\affiliation[\instGifu]{Gifu University, Gifu 501-1193, Japan}
\affiliation[\instSOKENDAI]{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\affiliation[\instMainz]{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\affiliation[\instGyeongsang]{Gyeongsang National University, Jinju 52828, South Korea}
\affiliation[\instHanyang]{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
%%%\affiliation[\instHeidelberg]{Heidelberg University, 68131 Mannheim, Germany}
\affiliation[\instHNU]{Henan Normal University, Xinxiang 453007, China}
\affiliation[\instKEK]{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\affiliation[\instJPARC]{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
%%%\affiliation[\instHiroshima]{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\affiliation[\instHUNNU]{Hunan Normal University, Changsha 410081, China}
%%%\affiliation[\instIKERBASQUE]{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao, Spain}
\affiliation[\instFrascati]{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\affiliation[\instNapoliINFN]{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\affiliation[\instPadovaINFN]{INFN Sezione di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaINFN]{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaINFN]{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreINFN]{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoINFN]{INFN Sezione di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteINFN]{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIISER]{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\affiliation[\instIITBhubaneswar]{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\affiliation[\instIITGuwahati]{Indian Institute of Technology Guwahati, Assam 781039, India}
\affiliation[\instIITHyderabad]{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\affiliation[\instIITJodhpur]{Indian Institute of Technology Jodhpur, Jodhpur 342030, India}
\affiliation[\instIITMadras]{Indian Institute of Technology Madras, Chennai 600036, India}
\affiliation[\instIndiana]{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\affiliation[\instIHEPRussia]{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\affiliation[\instHEPHYVienna]{Institute of High Energy Physics, Vienna 1050, Austria}
\affiliation[\instIHEPChina]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
%%%\affiliation[\instChennai]{Institute of Mathematical Sciences, Chennai 600113, India}
\affiliation[\instIPP]{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\affiliation[\instIOP]{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\affiliation[\instIFIC]{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\affiliation[\instISU]{Iowa State University, Ames, Iowa 50011, U.S.A.}
\affiliation[\instJAEA]{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
%%%\affiliation[\instJLU]{Jilin University, Changchun 130012, China}
\affiliation[\instKarlsruhe]{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\affiliation[\instKitasato]{Kitasato University, Sagamihara 252-0373, Japan}
\affiliation[\instKISTI]{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\affiliation[\instKoreaUnivKU]{Korea University, Seoul 02841, South Korea}
%%%\affiliation[\instKSU]{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\affiliation[\instKyotoU]{Kyoto University, Kyoto 606-8501, Japan}
\affiliation[\instKyungpook]{Kyungpook National University, Daegu 41566, South Korea}
\affiliation[\instLNNU]{Liaoning Normal University, Dalian 116029, China}
\affiliation[\instGiessen]{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\affiliation[\instLuther]{Luther College, Decorah, Iowa 52101, U.S.A.}
\affiliation[\instMNITJaipur]{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\affiliation[\instLMU]{Ludwig Maximilians University, 80539 Munich, Germany}
\affiliation[\instMcGill]{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
%%%\affiliation[\instMETU]{Middle East Technical University, 06531 Ankara, Turkey}
%%%\affiliation[\instMEPhI]{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\affiliation[\instNagoya]{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
%%%\affiliation[\instNagoyaIAR]{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNagoyaKMI]{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
%%%\affiliation[\instNNU]{Nanjing Normal University, Nanjing 210023, China}
%%%\affiliation[\instNankai]{Nankai University, Tianjin 300071, China}
\affiliation[\instNaraWu]{Nara Women's University, Nara 630-8506, Japan}
%%%\affiliation[\instUNAM]{National Autonomous University of Mexico, Mexico City, Mexico}
\affiliation[\instHSE]{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\affiliation[\instNTUTaiwan]{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
%%%\affiliation[\instNUUTaiwan]{National United University, Miao Li 36003, Taiwan}
\affiliation[\instKrakow]{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\affiliation[\instNiigata]{Niigata University, Niigata 950-2181, Japan}
\affiliation[\instNSU]{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
%%%\affiliation[\instOkinawa]{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\affiliation[\instOsakaMetropolitan]{Osaka Metropolitan University, Osaka 558-8585, Japan}
\affiliation[\instRCNP]{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\affiliation[\instPNNL]{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\affiliation[\instPanjab]{Panjab University, Chandigarh 160014, India}
%%%\affiliation[\instPeking]{Peking University, Beijing 100871, China}
\affiliation[\instMPP]{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
%%%\affiliation[\instMPGHLL]{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
%%%\affiliation[\instPanjabPAU]{Punjab Agricultural University, Ludhiana 141004, India}
\affiliation[\instRIKENMSL]{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\affiliation[\instSeoul]{Seoul National University, Seoul 08826, South Korea}
\affiliation[\instShandong]{Shandong University, Jinan 250100, China}
\affiliation[\instKyiv]{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\affiliation[\instSPU]{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\affiliation[\instSoochow]{Soochow University, Suzhou 215006, China}
\affiliation[\instSoongsil]{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\affiliation[\instSEU]{Southeast University, Nanjing 211189, China}
\affiliation[\instLjubljanaJSI]{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\affiliation[\instSKKU]{Sungkyunkwan University, Suwon 16419, South Korea}
\affiliation[\instTata]{Tata Institute of Fundamental Research, Mumbai 400005, India}
\affiliation[\instTUM]{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\affiliation[\instTelAviv]{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\affiliation[\instToho]{Toho University, Funabashi 274-8510, Japan}
%%%\affiliation[\instTohoku]{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\affiliation[\instTitech]{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\affiliation[\instTokyoMetropolitan]{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\affiliation[\instUAS]{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\affiliation[\instNapoliUNIV]{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\affiliation[\instPadovaUNIV]{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaUNIV]{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaUNIV]{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreUNIV]{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoUNIV]{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteUNIV]{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
%%%\affiliation[\instMontreal]{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\affiliation[\instIJCLab]{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[\instIPHC]{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\affiliation[\instAdelaide]{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
%%%\affiliation[\instBilbao]{Department of Physics \& EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao, Spain}
\affiliation[\instBonn]{University of Bonn, 53115 Bonn, Germany}
\affiliation[\instUBC]{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\affiliation[\instCincinnati]{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\affiliation[\instFlorida]{University of Florida, Gainesville, Florida 32611, U.S.A.}
%%%\affiliation[\instHamburg]{University of Hamburg, 20148 Hamburg, Germany}
\affiliation[\instHawaii]{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\affiliation[\instLjubljanaUniLJ]{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\affiliation[\instLouisville]{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
%%%\affiliation[\instMalaya]{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\affiliation[\instManitoba]{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\affiliation[\instLjubljanaUM]{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\affiliation[\instMelbourne]{School of Physics, University of Melbourne, Victoria 3010, Australia}
\affiliation[\instMississippi]{University of Mississippi, University, Mississippi 38677, U.S.A.}
%%%\affiliation[\instUOM]{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\affiliation[\instNovaGorica]{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\affiliation[\instUPES]{University of Petroleum and Energy Studies, Dehradun 248007, India}
\affiliation[\instPittsburgh]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
%%%\affiliation[\instUSTC]{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\affiliation[\instSAlabama]{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
%%%\affiliation[\instSCarolina]{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\affiliation[\instSydney]{School of Physics, University of Sydney, New South Wales 2006, Australia}
%%%\affiliation[\instTabuk]{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\affiliation[\instUTokyo]{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\affiliation[\instEri]{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\affiliation[\instIPMU]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\affiliation[\instVictoria]{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\affiliation[\instUppsala]{Uppsala University, SE-751 05 Uppsala, Sweden}
\affiliation[\instVPI]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\affiliation[\instWayneState]{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\affiliation[\instXavier]{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\affiliation[\instYamagata]{Yamagata University, Yamagata 990-8560, Japan}
\affiliation[\instYonsei]{Yonsei University, Seoul 03722, South Korea}
%%%\affiliation[\instZZU]{Zhengzhou University, Zhengzhou 450001, China}

==> definitions.tex <==
% Packages
\usepackage{graphicx} % Include figure files
\usepackage{epstopdf} % Allow to include eps files
\usepackage{dcolumn} % Align table columns on decimal point
\usepackage{xcolor} % Color support
\usepackage{amssymb} % Extended symbol collection
\usepackage{hyperref} % Generate pdfs with hyperlinks
\usepackage[utf8]{inputenc} % Allow UTF8 characters
\usepackage[english]{babel} % All publications are in English
%\usepackage[displaymath, mathlines]{lineno} % Line numbers for drafts
\usepackage{blindtext} % For testing
\usepackage{bashful}
\usepackage{siunitx}
\usepackage[italic]{hepnames}
\usepackage{caption}
%\captionsetup{justification = raggedright, singlelinecheck = false}
\captionsetup{font=small, justification = raggedright, singlelinecheck = false}              
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{tabularx}
\usepackage{amsmath}
\usepackage{orcidlink} % for ORCIDs in author list
\usepackage{lineno}
% Configuration


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace}
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%% \num conflicts with siunitx
% \def\num        {\ensuremath{\nu_\mu}\xspace}
% \def\numb       {\ensuremath{\nub_\mu}\xspace}
% \def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}
\def\Ddoublestar {\ensuremath{D^{**}}\xspace}
\def\Dzstar  {\ensuremath{D_{0}^{*}}\xspace}
\def\Done  {\ensuremath{D_{1}}\xspace}
\def\Doneprime  {\ensuremath{D'_{1}}\xspace}
\def\Dtwostar  {\ensuremath{D_{2}^{*}}\xspace}

\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

%%%%%%%%%%%%%%%%
%% R(Xemu) analysis
%%%%%%%%%%%%%%%%

% define own units for siunitx
% barn was built-in but is deprecated in latest siunitx versions, so we have to define it ourselves
\DeclareSIUnit\clight{\text{\ensuremath{c}}}
\DeclareSIUnit\barn{b}
\DeclareSIUnit\b{\barn}
\DeclareSIUnit\fb{\femto\barn}
\DeclareSIUnit\invfb{\per\femto\barn}
\DeclareSIUnit\ab{\atto\barn}
\DeclareSIUnit\invab{\per\atto\barn}
\DeclareSIUnit\gev{\GeV}
\DeclareSIUnit\gevc{\GeV\per\clight}
\DeclareSIUnit\gevcc{\GeV\per\clight\squared}


% General stuff
\newcommand*{\btag}{\ensuremath{B_\text{tag}}\xspace}
\newcommand*{\bsig}{\ensuremath{B_\text{sig}}\xspace}
\newcommand{\pell}{\ensuremath{p_{\ell}^{B}}\xspace}
\newcommand*{\plab}{\ensuremath{p^{\mathrm{lab}}}\xspace}
\newcommand*{\thetalab}{\ensuremath{\theta^{\mathrm{lab}}}\xspace}
\newcommand{\sigprob}{\ensuremath{\mathcal{P}_\text{FEI}}\xspace}
\newcommand{\mbc}{\ensuremath{M_{\textrm{bc}}}\xspace}
\newcommand{\deltae}{\ensuremath{\Delta E}\xspace}
\newcommand{\lumion}{\ensuremath{\SI{189}{\per\femto\barn}}\xspace}
\newcommand{\lumioff}{\ensuremath{\SI{18}{\per\femto\barn}}\xspace}
\newcommand{\FEI}{\texttt{FEI}\xspace}
% R ratios and branching fractions.
\newcommand{\RXemu}{\ensuremath{R(X_{e/\mu})}\xspace}
\newcommand{\RXemufid}{\ensuremath{R(X_{e/\mu}\mid p_{\ell}^{B}>1.3\,\gevc)}\xspace}
\newcommand{\BtoXtaunu}{\ensuremath{B\to \, X \, \tau \, \nu}\xspace}
\newcommand{\BtoXellnu}{\ensuremath{B\to X \, \ell \, \nu}\xspace}
\newcommand{\BtoXenu}{\ensuremath{B\to X \, e \, \nu}\xspace}
\newcommand{\BFXenu}{\ensuremath{\mathcal{B}(\BtoXenu)}\xspace}
\newcommand{\BtoXmunu}{\ensuremath{B\to X \, \mu \, \nu}\xspace}
\newcommand{\BFXmunu}{\ensuremath{\mathcal{B}(\BtoXmunu)}\xspace}
\newcommand*{\xclnu}{\ensuremath{X_c \, \ell \, \nu}\xspace}
\newcommand{\btoclnu}{\ensuremath{b \to c \, \ell \, \nu}\xspace}
\newcommand{\btoulnu}{\ensuremath{b \to u \, \ell \, \nu}\xspace}
% D, D* modes
\newcommand{\bdlnu}{\ensuremath{B \to D \, \ell\,\nu}\xspace}
\newcommand{\bdslnu}{\ensuremath{B \to D^* \, \ell\,\nu}\xspace}
\newcommand{\bdanddslnu}{\ensuremath{B \to D^{(*)} \, \ell\,\nu}\xspace}
\newcommand{\bdenu}{\ensuremath{B \to D \, e\,\nu}\xspace}
\newcommand{\bdsenu}{\ensuremath{B \to D^* \, e\,\nu}\xspace}
\newcommand{\bdmunu}{\ensuremath{B \to D \, \mu\,\nu}\xspace}
\newcommand{\bdsmunu}{\ensuremath{B \to D^* \, \mu\,\nu}\xspace}
\newcommand{\bsdlnu}{\ensuremath{B_s \to D_s \, \ell\,\nu}\xspace}
\newcommand{\bsdslnu}{\ensuremath{B_s \to D^*_s \, \ell\,\nu}\xspace}
\newcommand{\bpDlnu}{\ensuremath{B^+ \to \overline D^0 \, \ell\,\nu}\xspace}
% D** modes
\newcommand{\bddslnu}{\ensuremath{B \to D^{**} \, \ell \,\nu}\xspace}
\newcommand{\bddsenu}{\ensuremath{B \to D^{**} \, e\,\nu}\xspace}
\newcommand{\bddsmunu}{\ensuremath{B \to D^{**} \, \mu\,\nu}\xspace}
\newcommand{\bdonelnu}{\ensuremath{B \to D_1 \, \ell\,\nu}\xspace}
\newcommand{\bdstwolnu}{\ensuremath{B \to D^*_2 \, \ell\,\nu}\xspace}
\newcommand{\bdszerolnu}{\ensuremath{B \to D^*_0 \, \ell\,\nu}\xspace}
\newcommand{\bdoneprimelnu}{\ensuremath{B \to D'_1 \, \ell\,\nu}\xspace}
\newcommand{\bdtwoSlnu}{\ensuremath{B \to D_{2S} \, \ell\,\nu}\xspace}
\newcommand{\bdstwoSlnu}{\ensuremath{B \to D^{*}_{2S} \, \ell\,\nu}\xspace}
% gap modes
\newcommand{\bdanddspipilnu}{\ensuremath{B \to D^{(*)}\,\pi\,\pi\,\ell\,\nu}\xspace}
\newcommand{\bdanddsetalnu}{\ensuremath{B \to D^{(*)}\,\eta\,\ell\,\nu}\xspace}
% LID calibration channels
\def\kspipi         {\ensuremath{K_{\rm S}^0\to\pi^+\pi^-}\xspace}
\def\jpsimumu       {\ensuremath{\jpsi \to \mup\mun}\xspace}
\def\jpsiee         {\ensuremath{\jpsi \to \ep\en}\xspace}
\def\jpsill         {\ensuremath{\jpsi \to \ell^+\ell^-}\xspace}
\def\eegamma        {\ensuremath{\ep\en \to \ep\en (\gamma)}\xspace}
\def\mumugamma      {\ensuremath{\ep\en \to \mup\mun\gamma}\xspace}
\def\llgamma        {\ensuremath{\ep\en \to \ell^+\ell^-(\gamma)}\xspace}
\def\eeee           {\ensuremath{\ep\en \to (\ep\en)\ep\en}\xspace}
\def\eemumu         {\ensuremath{\ep\en \to (\ep\en)\mup\mun}\xspace}
\def\eell           {\ensuremath{\ep\en \to (\ep\en)\ell^+\ell^-}\xspace}
\def\eepipi         {\ensuremath{\ep\en \to (\ep\en)\pi^+\pi^-}\xspace}
\def\dstardkpipi    {\ensuremath{D^{*+}\to D^0(\to K^-\pi^+)\pi^+}\xspace}
\def\taupair        {\ensuremath{\ep\en\to \tau^{\pm}(\text{1-prong})\tau^{\mp}(\text{3-prong})}\xspace}
% CS quantities
%\newcommand*{\scaleoffres}{\ensuremath{c_\textrm{off-res}}\xspace}
%\newcommand*{\ecmsoffres}{\ensuremath{\sqrt{s}_\textrm{off-res}}\xspace}
%\newcommand*{\ecmsonres}{\ensuremath{\sqrt{s}_{\FourS}}\xspace}


